Active Assessment of Prediction Services as Accuracy Surface Over Attribute Combinations

Our goal is to evaluate the accuracy of a black-box classification model, not as a single aggregate on a given test data distribution, but as a surface over a large number of combinations of attributes characterizing multiple test data distributions. Such attributed accuracy measures become important as machine learning models get deployed as a service, where the training data distribution is hidden from clients, and different clients may be interested in diverse regions of the data distribution. We present Attributed Accuracy Assay (AAA)--a Gaussian Process (GP)--based probabilistic estimator for such an accuracy surface. Each attribute combination, called an 'arm', is associated with a Beta density from which the service's accuracy is sampled. We expect the GP to smooth the parameters of the Beta density over related arms to mitigate sparsity. We show that obvious application of GPs cannot address the challenge of heteroscedastic uncertainty over a huge attribute space that is sparsely and unevenly populated. In response, we present two enhancements: pooling sparse observations, and regularizing the scale parameter of the Beta densities. After introducing these innovations, we establish the effectiveness of AAA in terms of both its estimation accuracy and exploration efficiency, through extensive experiments and analysis.

==> attic/analysis.tex <==
\newcommand{\ones}{\mathbb{1}}

\section{Analysis}
The Gaussian approximated posterior $q^*(f)$ obtained by Laplacian approximation is:

$$
q(f) = \mathcal{N}(f|\hat{f}, A^{-1})
$$
where $A=\nabla\nabla \text{log Pr}(f|X, y)|_{f=\hat{f}}$ and $\hat{f}=\arg\max_f\text{log Pr}(f|X, y)$. This is obtained by second-order Taylor approximation on logPr(f|X,y)\footnote{see \url{http://www.gaussianprocess.org/gpml/chapters/RW3.pdf} for more details}.
\begin{align}
    \text{log Pr}(f|X, y) &\propto \text{log Pr}(y|f) + \text{log Pr}(f|X)\nonumber\\
    &= \text{log Pr}(y|f) - \frac{1}{2}f^TK^{-1}f - \text{log }|K| - \frac{n}{2}\text{log }2\pi  
    \label{eqn:qf:opt}
\end{align}
The term $\frac{1}{2}f^TK^{-1}f$ in the optimization is similar to the RKHS norm: $\|f\|_{\mathcal{H}}$ or $\frac{1}{2}\alpha^TK\alpha$. 

The $\text{log Pr}(y|f)$ in optimization expression~\ref{eqn:qf:opt} does not have a closed-form expression with non-Gaussian likelihood. We instead, adopt a proxy objective shown below for the ease of analysis.

\begin{align}
    \hat{f} &= \arg\min_f \frac{1}{2} \|y - \sigma(f)\|^2 + \frac{1}{2}(\sigma(f)-\frac{\ones}{2})^TK^{-1}(\sigma(f)-\frac{\ones}{2})\\
    &\text{replace $\sigma(f)$ with $\mu$ with the additional constraint that $\mu\in [0, 1]$}\\
    &\text{Leads to a ridge regression problem with closed form solution}\\
    \mu &= (I+K^{-1})^{-1}(y + K^{-1}\frac{\ones}{2})
\end{align}

We generalize this to the case when we smooth the observations by a smoothing matrix, denoted S. The observations now are $Sy$ and the corresponding estimate values $S\mu$. This leads to the following solution. 

\begin{align}
    \hat{f} &= \arg\min_f \frac{1}{2}\|Sy-S\mu\|^2 + \frac{1}{2}(\sigma(f)-\frac{\ones}{2})^TK^{-1}(\sigma(f)-\frac{\ones}{2})\\
    \implies & \mu = (S^TS + K^{-1})^{-1}(S^TSy + \frac{1}{2}K^{-1})
\end{align}
Finally the predictor in terms of the estimated $\mu$ for any point x is $K_{xX}K_{XX}^{-1}\mu$.

\begin{align}
    \hat{f} = \arg\min_f \frac{1}{2}\|Sy-Sf\|^2 + \frac{1}{2}f^TK^{-1}f\\
    \nabla_f L = 0\\
    \implies S^TSf - S^TSy + K^{-1}f = 0\\
    \implies f = (S^TS + K^{-1})^{-1}S^TSy
\end{align}

The bias and variance is given by the following expressions, similar to the earlier work, we assume the covariates are fixed and only their corresponding values are varied. 
Denote $Q=S^TS$.

\begin{align}
    \text{bias}^{2} = \mathbb{E}_{x,\hat{y}\sim \mathcal{N}(0,L)}[\|y^*-\hat{K}K^{-1}(Q+K^{-1})^{-1}(Qy+K^{-1}\frac{\ones}{2})\|^2_2]\\
    \text{variance} = \mathbb{E}_{x}\mathbb{E}_{\mathcal{D}_T}[\|\hat{K}K^{-1}(Q+K^{-1})^{-1}Q(y-\bar{y})\|^2]
\end{align}
$\hat{y}$ denotes the values for all the inputs while $y$ denote the values only for the observations. 

==> attic/region.tex <==
\subsection{The MeanOut Pooling Strategy}

The limitation with eqn.~\eqref{eq:pointLL} is that when many arms are sparsely populated, their empirical mean accuracies are granular and near/at 0 or 1, so that it is attractive for the likelihood maximization to center $\bmean(\f_{\attarm})$ around the empirical expected correctness of $\attarm$, and tune $K_1$'s parameters to decouple influence from other arms.


Our proposed remedy is to factor eqn.~\eqref{eq:pointLL} into \emph{regions}, which are groups of arms having reasonably large number of instances.  For each arm $\attarm$ with limited support ($n_\attarm$ small), we group it with a fixed number of other arms chosen randomly.  Arms with sufficient  support are retained as singleton regions. \todo{Arms with sufficient support are assigned to a singleton region apart from being pooled}  Region creation policies are further studied in Section~\ref{sec:expt:regions}.
%We will compute the population-weighted mixture Beta distribution over a region, and generate $\rho$ from this mixture, 
%to refine eqn.~\eqref{eq:pointLL} as follows.
%
Let $R(\dseed)$ denote a set of regions defined over the labeled dataset.  A region $r$ consists of a subset of arms. 
We use $\iacc_r=\sum_{\attarm \in r}\sum_{i: A(\vx_i)=\attarm} \iacc_i$ to denote the total accuracy score in region $r$.  Let $n_r$ denote the total number of labeled examples in region~$r$.  Suppose $w_{\attarm,r}=\frac{n_\attarm}{n_r}$ denotes the fraction of the instances in $r$ that belong to arm $\attarm\in r$.  Note that $\sum_{\attarm \in r} w_{\attarm, r} =1$.  
For each region $r$, each instance in the region chooses an arm $\attarm$ from $\text{Multi}(w_{\bullet,r})$, accesses its accuracy $\rho_\attarm$, and uses it in a Bernoulli sample. This allows us to express the likelihood of data under regions as:
\begin{multline}
\Pr(\{(\attarm_i, c_i: i\in[I] \}|\f,\g) = \\
\int_{\vec\rho \in [0,1]^{|\attspace|} } \prod_{r \in R(\dseed)} \prod_{i\in r} 
\sum_{\attarm\in r}
w_{\attarm,r}  \rho_\attarm^{\iacc_i}(1-\rho_\attarm)^{1-\iacc_i} 
\left[\textstyle \prod_{\attarm \in \attspace}
\Beta(\rho_\attarm|\bmean(f_\attarm), \bscale(g_\attarm)) \right] \text{d}\vec\rho.
\label{eq:regionLL1}
\end{multline}
Here $\vec\rho$ is the vector of possible latent accuracies with one component for each arm.  Their joint distribution is the product of marginals for a given $\f,\g$.  Eqn.~\eqref{eq:regionLL1} can be simplified to:
\begin{multline}
\int_{\vec\rho} \prod_{r}
\left[\textstyle\sum_a  w_{\attarm,r}  \rho_a\right]^{\iacc_r} \left[1-\textstyle\sum_a w_{\attarm,r} \rho_a\right]^{n_r-\iacc_r} 
\left[\textstyle \prod_{\attarm \in \attspace}
\Beta(\rho_\attarm|\bmean(f_\attarm), \bscale(g_\attarm)) \right] \text{d}\vec\rho.
\label{eq:regionLL2}
\end{multline}
Thus, each region's accuracy is a weighted mixture of the sampled accuracy of arms in the region.  This accuracy is used to fit a binomial distribution over the observations $\{c_r,n_r\}$ in region $r$. Contrast this with the arm-level likelihood terms in eqn~\eqref{eq:pointLL}.  When the number of observations in an arm ($n_\attarm$) is small, instead of supervising the GP parameters with possibly unreliable accuracy scores $c_\attarm$, we pool that arm's observations into larger regions with more reliable and stable $c_r$ and $n_r$. This way the GPs can be kept away from problematic solutions where variance of sparse arms are underestimated.  
%The above expression can be computed by sampling the $\rho$ values from the Beta distributions of each arm.

%Note that no matter how a region is constructed, the constraint on $\bmean(\f_{\attarm})$ is consistent with observed accuracy.
%The hope is that, by replacing or supplementing singleton regions having only one arm, possibly with sparse occupancy, with larger regions 

% \iffalse
% \todo{@vp: can plug in your toy examples here}

% Consider the case when we have 3 arms of accuracy {\it 0.2, 0.8, 0.8}. If we have only 3 observations for the first arm and 60 observations for the other two, we expect to not overfit on the sparse observation of the first arm and represent its low support through high variance. The variance of the fitted posterior distribution using eqn.~\eqref{eq:pointLL} for each arm averaged over 5 runs is {\it 0.03, 0.03, 0.03}. Notice how the uncertainty of the first arm does not reflect its low support. We next discuss an algorithm which can fix this problem. 
% \todo{vp: added this para}

% Region loss makes use of an arm's support to assign responsibility of the arm in explaining its subsuming region's observation. An arm with lowest support will be assigned the lowest responsibility in all of its regions. This allows for an arm with low support to have larger uncertainty. In the simple case of three arms, the variance of the fitted posterior using eqn.~\ref{eq:regionLL}, using random pooling strategy discussed in the next section of width 2, is {\it 0.04, 0.02, 0.02}, fixing the earlier problem of low uncertainty of the first arm with point loss. \todo{vp: Added this para}
% \fi

\subsubsection{A synthetic experiment}
\label{sec:synthetic}
We present a simple toy setting to explain our motivation behind MeanOut pooling.  Consider two arms with gold accuracy values $\accgold_1$ and $\accgold_2$ where $\dseed$ contains $n_1,n_2$ instances with $\iacc_1,\iacc_2$ of them being ones.  Assume $n_2 \gg n_1$.  In MeanOut we impose loss only on arm subsets with a sufficient number of observations.  Thus, we would have an arm-level loss on $a_2$ and a region loss on $(a_1,a_2)$.  Since $n_2$ is large, the point loss of $a_2$ would ensure that $P(\rho|a_2)$ is sharply peaked around $\gamma_2$.  Let us see how the data likelihood changes with the mean $\bmean_1$ and scale $\bscale_1$ of arm  $a_1$.  We obtain
\begin{equation}
     \text{PointLL}= \log\int_\rho \rho^{\iacc_1}(1-\rho)^{n_1-\iacc_1}  \Beta(\rho|\bmean_1, \bscale_1)) \text{d}\rho
     \label{eq:point:toy}
\end{equation}    
whereas with MeanOut we get
\begin{multline}
 \text{MeanOutLL} = \log\int_\rho 
\left[\tfrac{n_1}{n_2+n_1}\rho + \tfrac{n_2}{n_2+n_1}\gamma_2\right]^{\iacc_1+\iacc_2}\\
\left[ 1-\tfrac{n_1}{n_2+n_1}\rho - \tfrac{n_2}{n_2+n_1}\gamma_2\right]^{n_1+n_2-\iacc_1-\iacc_2}
\hspace{-2em}
\Beta(\rho|\bmean_1, \bscale_1)  \text{d}\rho.
\label{eq:region:toy}
\end{multline}
Above we have dropped the likelihood on observations $(c_2,n_2)$ in both equations. Also, we assume that arm $a_2$'s distribution is collapsed to a point at $\gamma_2$.  We plot the value of PointLL and MeanOutLL as a function of $\bmean_1$ and $\bscale_1$ in Figure~\ref{fig:surface}.   We find that the log-likelihood function is much flatter with MeanOutLL than PointLL even though the mode of the two surfaces is the same.

\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[trim=2cm 1cm 2cm 1cm, clip, width=.47\hsize]{images/PointLL.png} &
\includegraphics[trim=2cm 1cm 2cm 1cm, clip, width=.47\hsize]{images/MeanOutLL.png}
\end{tabular}
\caption{The likelihood surface of $(\phi_1, \psi_1)$, the less populated arm, with PointLL (Eqn~\ref{eq:point:toy}) on the left and with MeanOut pooling (Eqn~\ref{eq:region:toy}) on the right. Here $n_1=2, c_1=1, \gamma_1=0.2, \gamma_2=0.8, n_2=5,c_2=n_2\gamma_2$. }
\label{fig:surface}
\end{figure}

Of course, in practice the GP would impose its own smoothing on the parameters $\bmean_1,\bscale_1$ which we have not shown in the figure.  However, that smoothing might have to be carefully balanced against the likelihood, a process that becomes harder as the learned surface has heteroscadicity. MeanOut provides a form of data adaptive label smoothing.  The sensitivity of the likelihood on parameters of arms with few observations is reduced without making any assumption on the relationship of the accuracy at different arms.  This allows the shared parameters to be trained by more confident observations, without totally suppressing the less confident ones.  

\subsubsection{Approximating Region Likelihood}
\label{sec:region:approx}
The region likelihood expression involves an expensive integration over the $\vec\rho$ vector across all arms.  We explored various methods of implementing it.  One option is to use sampling with the Gumbel softmax trick to estimate the likelihood.  Another option is to decouple the marginalization over $\rho$ for each region and then estimate either via sampling or simpler function approximations.  An approximation that worked best for us empirically was to represent each region's accuracy as a mixture of Beta-distributions of arms in that region.  Using this, we approximate eqn.~\eqref{eq:regionLL2} as:
\begin{align}
\prod_{r} \int_{\rho} 
\textstyle \rho^{\iacc_r} (1-\rho)^{n_r-\iacc_r}
\textstyle\sum_{\attarm \in r} w_{\attarm,r} 
\Beta(\rho_\attarm|\bmean(f_\attarm), \bscale(g_\attarm)) \text{d}\rho.
\label{eq:regionMM}
\end{align}

The integration of the $\rho$ over Beta-mixtures can be computed in closed form like in eqn.~\eqref{eq:pointLLSimple} as:
\begin{align}
\prod_{r} \sum_{\attarm \in r}
  w_{\attarm,r} 
   \tfrac{\text{B}(\bmean(\f_{\attarm})\bscale(\g_\attarm) + \iacc_r,   (1-\bmean(\f_{\attarm}))\bscale(\g_\attarm)  + n_r -\iacc_r) }{
\text{B}(\bmean(\f_{\attarm})\bscale(\g_\attarm),   (1-\bmean(\f_{\attarm}))\bscale(\g_\attarm))
}
\label{eq:regionMM2}
\end{align}
The above expression may give the impression that a sparse arm is unduly coerced to match the accuracy of a dense region, but the effect of multiple sampled regions is merely to create enough confusion that the GP does not collapse on the unreliable empirical mean of the sparse arm.

We present an empirical comparison of different approximation methods in supplementary material.  In the main paper we compare the above MeanOut region likelihood with per-arm likelihood in eqn.~\eqref{eq:pointLLSimple}.

%We therefore approximate the expression by decoupling the integration for each region.


